Experimental determination of axion signal power of dish antennas and dielectric haloscopes using the reciprocity approach

The reciprocity approach is a powerful method to determine the expected signal power of axion haloscopes in a model-independent way. Especially for open and broadband setups like the MADMAX dielectric haloscope the sensitivity to the axion field is difficult to calibrate since they do not allow discrete eigenmode analysis and are optically too large to fully simulate. The central idea of the reciprocity approach is to measure a reflection-induced test field in the setup instead of trying to simulate the axion-induced field. In this article, the reciprocity approach is used to determine the expected signal power of a dish antenna and a minimal dielectric haloscope directly from measurements. The results match expectations from simulation but also include important systematic effects that are too difficult to simulate. In particular, the effect of antenna standing waves and higher order mode perturbations can be quantified for the first time in a dielectric haloscope.

==> dump.tex <==
%In term of fields it can be defined on the reference plane $S_T$ as 
%\begin{equation}
 %   \Gamma = \frac{\int_{S_T} \dd{A} \vb*{E} \cdot \vb*{E}^*_{\mathrm{in}}}{\int_{S_T} \dd{A} \left\lvert\vb*{E}_{\mathrm{in}}\right\rvert^2} -1. 
 %   \label{Eq:gamma_def}
%\%end{equation}
%The input field $\vb*{E}_{\mathrm{in}}$ is generated by the VNA with input power $P_{\mathrm{in}}$ whereas $\vb*{E}$ is the total field including reflections. 


%The Hermite-Gaussian mode content of the measured beam is quantified by the overlap integral between ${E}$ and fitted ${E}_{ml}$,

%\begin{equation}
%    \eta_{ml} = \frac{\left\lvert \int \dd{A} {E} \vdot {E}_{ml} \right\rvert^2}{\int \dd{A} \left\lvert {E} \right\rvert^2 \int \dd{A} \left\lvert {E}_{ml} \right\rvert^2}.
%    \label{Eq:eta_ml}
%\end{equation}

%The fundamental mode content $\eta_{00}$, figure \ref{fig:no_booster_eta_g_freq}, is found to be $>\SI{97}{\percent}$. 





%Using the thin lens equation one can calculate $w_0$ from the beam waist size $w_A$ and position $z_A$ of the antenna 
%\begin{equation}
%    w_A^2 = w_0^2 \frac{z_A - f}{z_0 - f},
%\end{equation}
%where $f$ focal length of the focusing mirror. Both $w_A$ and $z_A$ where measured independently in a reverberation chamber (todo check) while $f$ is known from focusing mirror geometry. The expected $w_0$ The comparison between the reverberation chamber measurement of $w_A$ and bead pull measurement can be seen in figure \ref{fig:no_booster_wA}. 


%The mode content $\eta_{ml}$ is shown in figure \ref{fig:mirror_eta_ml} for the fundamental mode and the sum of all HoM. The waist parameters from the antenna beam measurements were used to define ${E}_{ml}$. The matching to the fundamental mode $\eta_{00}$ closely resembles $\left\lvert\Gamma\right\rvert$. This can be understood from the similarity between the definition of $\Gamma$ \eqref{Eq:gamma_def} and $\eta_{ml}$ \eqref{Eq:eta_ml} if ${E}_{\mathrm{in}}={E}_{00}$. It is effectively a re-calibration of the reference plane $S_T$ from the input connector of the antenna to a transverse plane in front of the plane mirror. This opens up the interesting possibility of de-embedding the antenna and focusing mirror and simplifying the analysis. As this article is about validating the reciprocity approach and not about understanding all the intricacies of a dielectric haloscope, the apparent match between $\Gamma$ and $\eta_{00}$ serves, for now, just as another consistency check of the experimental method. It is, in fact, the strength of the reciprocity approach that one does not need to know anything about the setup as long as one can measure ${E}$, integrate and obtain the axion signal power $P_{\mathrm{sig}}$.   



%The overlap $\eta_A$ is defined as

%\begin{equation}
%    \eta_A = \frac{\left\lvert \int \dd{A} {E} a {B}_e \right\rvert^2}{\int \dd{A} \left\lvert {E} \right\rvert^2 \int \dd{A} \left\lvert a {B}_e \right\rvert^2}.
%\end{equation}
%A uniform $a {B}_e$ truncated at the radius of the disk is assumed for simplicity.\footnote{The contributions of non-zero ${E} \vdot a {B}_e$ for $r>r_D$ can be neglected since ${E}$ is well constrained by $w_0 \ll r_D$} In figure \ref{fig:mirror_formfactor}, $\eta_A$ is shown over frequency for the dish antenna setup as well as the expectation from the measured antenna beam of the previous section. The antenna-booster resonances lead to a deviation of $\eta_A$ from expectation of up to $\SI{78}{\percent}$. Generally, $\eta_A$ depends on $z$ as the waist size changes with $w(z)$. This is indicated by the the ribbon in figure \ref{fig:mirror_formfactor}. The relative change is less than todo which indicates that the beam shape is relatively constant over measured $z$, as expected from a Rayleigh range of $\sim \SI{30}{\centi \metre}$. 


\section{Detailed description of setup}


\subsection{Experiment}

\subsubsection*{Booster}
The dielectric disk and plane mirror have a diameter of $\SI{300}{\milli\metre}$ and are separated by a distance of $\SI{8.2}{\milli\metre}$. The dielectric disk has a thickness of $\SI{1}{\milli \metre}$ and is made out of sapphire which has a relative permittivity of $\epsilon \sim 9.3$ along its radial direction. The plane mirror is $\SI{3}{\milli\metre}$ thick and made from aluminium. These dimensions lead to a resonance frequency of $\nu_0 \sim \SI{19}{\giga \hertz}$. Geometric inaccuracies like tilts and surface deformation can have a large effect on the overall signal power (cite knirck). The distance to the plane mirror is set mechanically by spacers. From mechanical tolerances, the tilt between disk and mirror is estimated to be less than $\gamma < \SI{1}{\milli \radian}$. Planarity of the disk is measured to be TODO while for the mirror it is TODO. 

\subsubsection*{Focusing mirror}
The focusing mirror is an off-axis ellipsoidal mirror with a focal length of $f=\SI{352.47}{\milli \metre}$ and reflection angle of $\SI{60}{\deg}$. It was machined from a $\SI{387}{\milli\metre} \times \SI{335}{\milli\metre}$ aluminium (todo alloy) block. The maximum deviation from the ideal shape was measured to be less than $\SI{30}{\micro \metre}$. The distance between its reflection point and plane mirror is $d_2 = \SI{700}{\milli\metre}$(todo). The distance to the antenna aperture is $d_1 = \SI{350}{\milli\metre}$(todo).

\subsubsection*{Antenna}
The antenna is a corrugated circular horn antenna designed by the Max Planck Institute for Radio Astronomy. It is optimized for operation between $\SI{18}{\giga\hertz}$ and $\SI{26.5}{\giga\hertz}$ with a return loss, gain, insertion loss, cross polarization todo. Its output is a near perfect gaussian beam with a waist size of $w_0^1=\SI{25.61}{\milli\metre}$ at $\SI{22}{\giga\hertz}$ (todo at 19 ghz). 

\subsubsection*{VNA}
The VNA is a Rhode and Schwarz ZVA67. Dynamic range, cables, etc, calibration

\subsubsection*{Bead pull system}
The alumina bead has a radius $R=\SI{1.5}{\milli\metre}$ and permittivity $\epsilon \sim 9.7$. It is attached to a string made from high-modulus polyethylene with diameter of $\SI{0.1}{\milli\metre}$. The bead can be positioned in three dimensions by stepper motors. 
